Discrete Monodromy, Pentagrams, and the Method of Condensation

This paper considers a simple geometric construction, called the Pentagram map. The pentagram map, performed on N-gons, gives rise to a birational mapping on the space of all N-gons. This paper finds what conjecturally are all the invariants for this map, and along the way relates the construction to the monodromy of 3rd order differential equations, and also to Dodgson's method of condensation for computing determinants.

==> 2ell.tex <==

\section{The Proof}


==> 7rec.tex <==

\section{Proof of Theorem \ref{hyper}}

\subsection{Degenerate polygons}

We fix $n=4m$.   To avoid trivial cases, we assume
that $m$ is large$-$say, $m \geq 3$.  We work
over $\C$.  Everything we do is understood to
be defined for the generic example, but
perhaps not for every example.  
The reader should insert this caveat before
every assertion.
We will work with PolyPoints
and PolyPoints which are periodic mod $n$.
By this we mean that the points or lines
themselves are periodic, not just the
projective invariants.  We will call such
objects {\it periodic PolyPoints\/} or
{\it periodic PolyLines\/}.  We take these
to be elements of the spaces $P_1$ and $L_1$
introduced in \S 5.1.

We say that the periodic PolyPoint $A=\{...A_1,A_5,...\}$ is
{\it degenerate\/} if $...A_1,A_9,A_{13}...$ lie
on the same line and if $...A_3,A_{11},A_{15},...$ all
lie on the same line.  We make the dual definition
for PolyLines.  A polygon (in the ordinary sense)
satisfying the hypothesis of Theorem \ref{hyper}
naturally determines a degenerate PolyLine.
One simply considers the lines considered by the
edges of the polygon.

\begin{lemma}
\label{recip}
A periodic element in $P_1$ is degenerate iff
its projective invariants satisfy $q_jp_{j+1}=1$
for all $j$.  Dually, a periodic element in $L_1$
is degenerate if and only if its projective
invariants satisfy $p_jq_{j+1}=1$ for all $j$.
\end{lemma}

\startproof
By duality it suffices to prove this result for
PolyPoints.  Referring to the PolyPoint constructed
in \S 4, we compute
$$\det(A_{-1},A_5,A_{13})=p_1(1-q_2p_3).$$
The three points in question lie on the same
line iff $q_2p_3=1$.  By symmetry, similar
statements hold for other triples of points.
\endproof


\begin{lemma}
\label{closed}
If $A$ is a periodic $2n$-gon then
$$(\sum_{k=0}^{[n/2]} O_k)^3=27 O_n^2E_n; \hskip 15 pt
(\sum_{k=0}^{[n/2]} E_k)^3=27 E_n^2O_n.$$
\end{lemma}

\startproof
This is a corollary of Theorem
\ref{monodrom}. If
$A$ is $2n$-periodic then its monodromy
$T$ is the identity.  Likewise,
$T^*$ is the identity matrix.
Hence $\Omega_1=\Omega_2=27$.
\endproof

For Theorem \ref{hyper} we only
need the second statement of the next result.
The spaces $P_1$ and $L_1$ are defined in
\S 5.1.

\begin{lemma}
\label{van}
A degenerate element in either $P_1$ or $L_1$
has pentagram invariants \begin{enumerate}
\item $O_k=E_k=0$ for $k<2m$ and 
\item $O_{2m}=E_{2m}=2$ and
$O_n=E_n=1$.
\end{enumerate}
\end{lemma}

\startproof
First suppose that $k<2m=n/2$.  Using
the reasoning in the proof of Theorem \ref{trans} we
can group
$O_k$ into pieces having the form
$\prod \mu$, where each $\mu$ is a monomial
times  $(1-q_jp_{j+1})$ for some $j$.
(Compare Lemma \ref{seq2}, but interchange
$p$ with $q$.)
By Lemma \ref{recip} each $\mu$ is zero
and hence $O_k=0$.  The same argument
works for $E_k$.

We now turn to the second item.
Note that $$O_nE_n=(p_2q_3)(p_4q_5)...=(1)(1)...=1.$$
It now follows from Lemma \ref{later}
that $E_n^2=O_n^2=1$.   If $O_n=-1$, for any particular
example, then by continuity
$O_n$ is identically $-1$.  However, we
can choose a $4n$-point, contained in $\R^2$, which is essentially
the double cover of a $2n$-point.  The
invariants of such a $4n$-point would
repeat with period $2n$, forcing $O_n$ to be
a square of a real number.  This rules
out the possibility that $O_n=-1$.  Hence
$O_n=1$ for every example.  Likewise
$E_n=1$ for every example.
If now follows from Corollary \ref{closed},
and from the vanishing of all the other
pentagram invariants, that
\begin{equation} \label{closed2}
1+O_{2m}=3O_n=3; \hskip 30 pt
1+E_{2m}=3E_n=3. \end{equation}
Hence $E_{2m}=O_{2m}=2$.
\endproof

\subsection{The Main Argument}

We start with a degenerate PolyLine.  This
PolyLine determines a labelling of a single
row of 
the triangulation $\tau$, considered in \S 6.
Combining Theorem
\ref{lift} and Lemma \ref{van} we see that
we can find a circulent condensation $C$
which translates into our pentagram labelling.

\begin{center}
\psfig{file=Pix/pix65.ps}
Figure 6.5
\end{center}


Referring to the proof of Theorem \ref{lift} we
can use the fact that $p_jq_{j+1}=1$ to arrange
so that $r_jr_{j+1}=1$ for all $j$.  This allows
to pick our $c$ labelling so that the row below the
edge labels is identically $1$, as shown in
Figure 6.5.  Figure 6.5 is supposed to be periodic
in the horizontal direction.

We pull our $c$ labelling back to give a labelling of
$T$, the tiling of $\R^3$ by  octahedra.
The bottom row of dots pulls back to an infinite
horizontal plane of dots labelled by $1$.  The next layer up
pulls back to give the labelling of the next
horizontal plane, as shown in Figure 6.6.
This labelling is periodic with respect to
horizontal and vertical translation by $n$.
Each $n \times n$ block is a circulent matrix.
For generic choice of variables, this
circulent matrix will have nonzero determinant.

\begin{center}
\psfig{file=Pix/pix66.ps}
Figure 6.6
\end{center}


When we develop the condensation upwards, we
arrive precisely at a sandwich condensation of
width $n$.   Going back to the planar picture,
we see that the $n$th horizontal row of our
vertex labelling is a constant labelling,
as shown in Figure 6.7.

\begin{center}
\psfig{file=Pix/pix67.ps}
Figure 6.7
\end{center}

Since the top later of vertices is all constant, the
layer of edges directly below it must have labels
$s_1,t_2,s_3,t_4...$ where $t_2=1/s_1$, $t_4=1/s_3$, etc. 
By Lemma \ref{recip} the PolyPoint corresponding
to this row is degenerate.  That is, the vertices
of this PolyPoint lie on a pair of lines.
Translating this information back into the
language of the pentagram map, we see that
it corresponds exactly to the statement
of Theorem \ref{hyper}.

\newpage


==> 8vanish.tex <==



==> extra <==

\subsection{Poncelet Polygons}

In this section we will investigate how the pentagram
map and the pentagram invariants interact with
conic sections.  We suppose
that $p_1,q_2,...,q_{2n}$ are the projective
invariants of $A \in P_1$.

\begin{lemma}
\label{conic1}
 Suppose $A$ is inscribed in a conic.
Then 
$$(1-q_{2k})(1-q_{2k-2}p_{2k-1})=
(1-p_{2k-1})(1-q_{2k}p_{2k+1});$$ $$
(1-p_{2k-1})q_{2k}(1-p_{2k+1})=
(1-q_{2k-2})p_{2k-1}(1-q_{2k})$$
for $k=1,...,n$.  Here indices are
taken mod $2n$.
\end{lemma}

\startproof
We will derive the first identity.  The second
one is a fairly straightforward rearrangement
of the first.   Figure 5.2 shows an application
of Pascal's theorem.  If the $6$ points
$A_{-3},A_1,A_5,A_9,A_{13},A_{17}$ lie on a
conic section then the points
$C_1,C_2,C_3$ lie on a line.


\begin{center}
\psfig{file=Pix/pix52.ps}
Figure 5.2
\end{center}

If we express the $C_j$ in homogeneous coordinates,
we have \begin{eqnarray}
C_1=(A_{-3} \times A_{13}) \times (A_1 \times A_9) \cr \cr
C_2=(A_{-3} \times A_{17}) \times (A_5 \times A_9) \cr \cr
C_3=(A_{5} \times A_{13}) \times (A_1 \times A_{17})
\end{eqnarray}

The condition that the $C$s lie on the same line is
given by
\begin{equation}
\label{det}
\det(C_1,C_2,C_3)=0.
\end{equation}
In other words, we arrange these vectors into
a $3 \times 3$ matrix and set the determinant
equal to $0$.  

When we do this calculation on Mathematica, we see that
Equation \ref{det} holds if and only if
$(1-q_4)(1-q_2p_3)=(1-p_3)(1-q_4p_5).$  If all points
of $A$ lie on the same conic, then by symmetry the
same relation holds with the indices shifted
by $2,4,6...$
This completes our proof.
\endproof

From duality we get

\begin{corollary}
\label{conic2}
Suppose the $A^*$ is inscribed in a conic.
Then $$(1-q_{2k})(1-q_{2k+2}p_{2k+1})=
(1-p_{2k+1})(1-q_{2k}p_{2k-1});$$ $$
(1-p_{2k-1})q_{2k}(1-p_{2k+1})=
(1-q_{2k+2})p_{2k+1}(1-q_{2k})$$
for $k=1,...,n$.  Here indices are
taken mod $2n$.
\end{corollary}

For later use we record

\begin{corollary}
\label{later}
If $A$ is inscribed in a conic then
$O_n(A)=E_n(A)$.
\end{corollary}

\startproof
Taking the product of the first equation over all
$k$, and cancelling terms, we see that
$\prod (1-p_{2k-1})=\prod (1-q_{2j})$.
Taking the product of the second equation,
over all $k$, we get
$O_n (\prod (1-q_{2k})^2=
E_n (\prod (1-p_{2k-1})^2$.
Using the first equation to cancel terms,
we are left with $O_n=E_n$.
\endproof


We now turn to the proof of Theorem \ref{ponc}.
We will suppose that $A \in P_1$ is inscribed in a conic
section and the dual $A^*$ is also inscribed
in a conic section.  We will then show that
the projective invariants of $A$ are the
same as those of $\alpha_j(A)$ for $j=1,2$.
This is a completely equivalent formulation
of the first half of Theorem \ref{ponc}.

Let $q_1',p_2',...,p_{2n}'$ be the coordinates
of $\alpha_1(A)$. 
A special case of Corollary \ref{conic2} says that
\begin{equation}
\label{rel}
1-p_1q_2=\frac{(1-q_2)(1-p_3q_4)}{1-p_3}; \hskip 15 pt
1-p_5q_6=\frac{(1-p_5)(1-p_3q_4)}{1-q_4}.
\end{equation}
From Equation \ref{basic} we have
$$q'_3=q_4 \frac{1-p_5q_6}{1-p_1q_2}=
q_4 \frac{(1-p_3)(1-p_5)}{(1-q_2)(1-q_4)}=p_3.$$
The last equality is Lemma \ref{conic1}.
We now know that $q'_3=p_3$.  It follows
from the dihedral symmetry of our constructions
that $q'_1=p_1$, $p'_2=q_2$, etc.
A similar argument gives the same result for
$\alpha_2$.

For the second part of the result,
suppose $P$ and $Q$ are co-Poncelet polygons.  Let
$E_1$ and $E_2$ be the defining conics.
We can choose an arbitrarily small perturbation
of $E_2$, called $F_2$, with the following
properties.  First, $F_2$ is a conic section.
Second, there is an infinite polygon $R$
inscribed in $E_1$ and circumscribed about
$F_2$.  Third, the vertices of $P$ are
dense in $E_1$. Some finite portion of $R$ is a
small perturbation of $P$ and another
finite portion is a small perturbation of $Q$.
The first part of Theorem \ref{ponc} works
for infinite polygons as well, so that
$R'$ is projectively equivalent to $R$.
Hence $R'$ is inscribed in a conic $E_1'$ and
circumscribed about a conic $F_2'$.  But 
a finite portion of $R'$ is a perturbation of
$P'$ and another finite portion is a perturbation
of $Q'$.  Hence $P'$ and $Q'$ are nearly
inscribed in $E_1'$ and nearly circumscribed
about $F_2'$.  Taking the limit of a sequence
of increasingly small perturbations we see
that $P'$ and $Q'$ are co-Poncelet.


==> intro.tex <==
!

